Monotonic Prefix Consistency in Distributed Systems

We study the issue of data consistency in distributed systems. Specifically, we consider a distributed system that replicates its data at multiple sites, which is prone to partitions, and which is assumed to be available (in the sense that queries are always eventually answered). In such a setting, strong consistency, where all replicas of the system apply synchronously every operation, is not possible to implement. However, many weaker consistency criteria that allow a greater number of behaviors than strong consistency, are implementable in available distributed systems. We focus on determining the strongest consistency criterion that can be implemented in a convergent and available distributed system that tolerates partitions. We focus on objects where the set of operations can be split into updates and queries. We show that no criterion stronger than Monotonic Prefix Consistency (MPC) can be implemented.

==> closure.tex <==
% !TEX root = main.tex

% \subsubsection{Partition Tolerance}

% The implementations we study are \emph{partition tolerant}, in the sense
% that they are deployed on a network that may delay messages arbitrarily.
% In the semantics of $\impl$, the only thing that we require for a receive 
% action is that there exists a corresponding broadcast action that happened
% before it. This means that messages may be reordered, duplicated, or 
% arbitrary delayed in the network.


% \subsubsection{Eventual Delivery}

% To avoid networks where the partitions are permanent, we define the notion
% of \emph{fair execution}. Intuitively, fair executions happen on networks
% where every message is \emph{eventually delivered}.
% An infinite execution of $\impl$ is called \emph{fair} if, for
% every broadcast action $(\aid,\pid,\send{\msgid,\msg})$, and for 
% every $\pid\,' \in \Pid$, there exists a
% corresponding receive action 
% $(\aid\,',\pid\,',\receive{\msgid,\msg})$ for some $\aid\,' \in \Nat$.
% Finite executions are considered fair by default.
% We denote by $\fair{\impl} \subseteq \semantics{\impl}$ be the subset of fair 
% executions of $\impl$.
% % We restrict the definition of $\semantics{\impl}$ in order to keep only 
% % fair executions.



% \subsubsection{Availability}

% We focus on implementations which are \emph{available}. 
% This means that client requests are always answered, regardless of what is 
% happening in the network. Formally, this is represented by the fact that 
% the handlers of client requests and incoming messages are computable functions,
% and by the fact that when defining the semantics of $\impl$, we allow for 
% client requests to happen at any time.


% \subsubsection{Safety and Convergence}

% Moreover, we focus on implementations that are \emph{safe} and 
% \emph{convergent}. These two notions are defined with respect to the 
% intended specification for the abstract object being implemented. 
% More specifically, we assume that we are given a \emph{specification}
% $\spec \subseteq (\Req \times \Ans)^*$, which is a set of sequences of 
% pairs of requests and answers, describing the valid sequential behaviors
% of the object.

% Specifications are \emph{input enabled}, meaning that for any run of the 
% specification, we can add an additional request $\req \in \Req$.
% Formally, for every $w \in \spec$, $\req \in \Req$, there exists 
% $\ans \in \Ans$ such that $w \cdot (\req,\ans) \in \spec$.
% Moreover, specifications are \emph{prefix closed}, meaning that for 
% any sequences $w_1 \cdot w_2 \in \spec$, we have $w_1 \in \spec$.

% Given a trace $\tr$, we denote by $\opsof{\tr}$ the set of action identifiers 
% of $\tr$.
% A trace $\tr$ is said to be \emph{safe} (with respect to $\spec$) if
% there exists $\vis \subseteq \opsof{\tr} \times \opsof{\tr}$ such that:
% \begin{itemize}
% \item if $\op_1 \ltvis \op_2$, then $\op_1$ is before $\op_2$ in $\vis$,
% \item 
%   for every action $(\aid,\pid,\req,\ans) \in \tr$, 
%   there exists $w \in \sequences{\completions{\vis^{-1}(\aid)}}$
%   such that $w \cdot (\req,\ans) \in \spec$.
% \end{itemize}
% In addition, a safe trace is \emph{convergent} if for every action 
% $\op \in \opsof{\tr}$, the set of operations for which $\op$ is not visible
% is finite, 
% \ie $\set{\op'\ |\ \op \not \ltvis \op'}$ is finite.

% For the rest of the paper, we restrict our attention to  implementations that 
% only produce safe and convergent traces.


==> eventual.tex <==
\section{Consistency Criterion}

\subsection{Notations}

Let $\Req$ be a set of requests and $\Ans$ be the domain of possible 
answers.
A \history{} $\hist$ is a poset $(\ops,\po,\flabel)$ labelled by 
$\Act$, where $\po$, the \emph{program order}, is a disjoint union of total
orders.
A specification $\spec$ is a set of sequences labelled by $\Act$.
The specification represents the set of valid sequences of an abstract 
object such as a stack, a queue, a key-value store, \dots

We denote by $\projectrv{\rho}{\ops'}$
the labelled poset where only the return values of the operations in
$\ops'$ have been kept.
Formally, $\projectrv{\rho}{\ops'}$ is
the $(\Req \times \Ans) \cup \Req$ labelled poset $(\ops,<,\getlabel')$ where
for all $\op \in \ops'$, $\getlabel'(\op) = \getlabel(\op)$,
and for all $\op \in \ops \setminus \ops'$, if
$\getlabel(\op) = (\meth,\rv)$, then
$\getlabel'(\op) = \meth$.
% Said differently $\projectrv{\rho}{\ops'}$ only keeps the return values
% of the 
If $\ops' = \set{\op}$, we denote
$\projectrv{\rho}{\ops'}$ by $\projectrv{\rho}{\op}$.


Second, we introduce a relation on labelled posets, denoted $\weaker$.
Let 
$\rho = (\ops,<,\getlabel)$ and 
$\rho' = (\ops,<',\getlabel')$ 
be two posets labelled by 
$(\Req \times \Ans) \cup \Req$ (the answers of some requests 
in $\ops$ might not be specified).
We denote by $\rho' \weaker \rho$
the fact that $\rho'$ has fewer order and label constraints on the set $\ops$.
Formally, $\rho' \weaker \rho$ if $<'\, \subseteq\, <$ and for all operation 
$\op \in \ops$, 
and for all $\meth \in \Req$, $\rv \in \Ans$,
\begin{itemize}
% \item $\op_1 <' \op_2$ implies $\op_1 < \op_2$, and either
%   \begin{itemize}
  \item $\getlabel(\op) = \getlabel'(\op)$, or 
  \item
    $\getlabel(\op) = (\meth,\rv)$ implies
    $\getlabel'(\op) = \meth$.
%   \end{itemize}
\end{itemize}
 
\begin{table}

\begin{tabular}{l|l}
    \axthinair & $\vis \cup \po$ is acyclic \\
    \axrv & 
        $\projectrv{\thepast{\op}}{\op} \weaker \loco$ \\
    \axmr &
        $\vis \circ \po \subseteq \vis$ \\ 
%  \axpf & $\go$ is prefix-founded \\
%  \axeventual & 
%   $\getprefix{\go}{r} \pref \loco$ for all 
%   $r \in \Nat$, $\getround(\op) > r + B$\\
 \axprefix & 
    $\loco \pref \go$ \\
 \axbounded  &
    $\op_1 \ltvis \op_2$ for all $\op_1,\op_2 \in \ops$ \\
    & 
    with $\getround(\op_1) + B < \getround(\op_2)$ 
\end{tabular}

\vspace{2em}
with:\\
$\vispast{\op} = \set{\op' \in \ops \ |\ \op' \leqrel{\vis} \op}$,\\
$\lasting{\op} = \set{(\op',\op) \ |\ \op' \ltrel{\vis} \op}$, \\
$\thepast{\op} = (\vispast{\op},\lasting{\op},\getlabel)$.
% $\getprefix{\go}{r}$ is the smallest prefix of $\go$ containing all 
% which were submitted before round $r$,\\
% $\getbefore{\ops}{r} \subseteq \ops$ is the set of operations 
% $\op'$ with $\getround(\op') \leq r$.\\
\caption{Axioms used in the definition of eventual consistency.}
\label{tab:axioms}
\end{table}

 
 
% \subsection{$B$-Eventual Consistency}
% 
% 
% \begin{definition}
% % Let $\bound: \Nat \rightarrow \Nat$ be a increasing function whose limit
% % at $+\infty$ is $+\infty$.
% Let $\bound \in \Nat$.
% The history $\hist = (\ops,\po,\flabel)$ is \emph{$\bound$-\eventually{} 
% ($\bound$-\ec{} for short)} with respect to a specification $\spec$
% if there exist a strict total order 
% $\go \subseteq \ops \times \ops$ 
% and a strict partial order $\vis \subseteq \ops \times \ops$ such that
% for every $\op \in \ops$
% there exists a sequence $\loco \in \spec$ satisfying
% the axioms \axthinair, \axrv, 
% \axeventual{} defined in 
% \tab{tab:axioms}. 
% \end{definition}
% 
% Axiom~\axthinair{} is due to physical constraints, as 
% $\op_1 \ltrel{\vis} \op_2$ intuitively means that operation $\op_1$ is 
% visible to operation $\op_2$.
% 
% Axiom~\axrv{} is a safety constraint, ensuring that the return value of $\op$
% is valid according to the specification $\spec$. More specifically, it
% ensures that the return value of $\op$ can be obtained by ordering the 
% operations visible to $\op$ in some order which respects the specification 
% $\spec$.
% 
% Formally, to define \axrv, we take the labelled poset $\thepast{\op}$, which
% orders all the operations visible to $\op$ before $\op$ itself, and
% project away all return values except $\op$'s.
% We then verify that the resulting labelled poset, 
% $\projectrv{\thepast{\op}}{\op}$,
% can be sequentialized into a sequence $\loco$ of the specification, that is
% $\projectrv{\thepast{\op}}{\op} \weaker \loco$.
% 
% Axiom~\axeventual{} ensures that \sites{} converge towards the same total 
% order $\go$. More specifically, for each round $r \in \Nat$, 
% and every operation $\op \in \ops$ with $\getround(\op) > r + B$, the order 
% $\loco$ must have $\getprefix{\go}{r}$ as a prefix -- where 
% $\getprefix{\go}{r}$ is defined as the smallest prefix of $\go$ which contains
% all operations that happened at round $r$ or before.


\subsection{Consistent Monotonic Prefixes}


% \begin{figure}
% % \begin{tikzpicture}
% % 
% \footnotesize
% \centering

% \begin{subfigure}[t]{0.22\textwidth}

% \centering
% \begin{minipage}[t]{0.4\textwidth}
% $\pid_a$:\\
% $\mkwrite{\var}{1}$\\ 
% $\mkread{\var}{1}$\\
% $\mkread{\var}{2}$\\
% $\mkread{\var}{1}$\\
% \end{minipage}
% \begin{minipage}[t]{0.2\textwidth}
% $\pid_b$:\\
% $\mkwrite{\var}{2}$\\
% \end{minipage}

% \caption{Eventually consistent and eventually linearizable, but not $B$-\cmp}
% \label{fig:elnotcmp}

% \end{subfigure}
% \begin{subfigure}[t]{0.22\textwidth}
% % 
% \centering
% \begin{minipage}[t]{0.4\textwidth}
% $p_a$:\\
% $\mkwrite{\var}{0}$\\
% $\mkwrite{\var}{1}$\\ 
% $\mkread{\var}{0}$\\
% $\mkread{\var}{1}$\\
% $\mkwrite{\var}{0}$\\
% $\mkwrite{\var}{1}$\\ 
% $\mkread{\var}{0}$\\
% $\mkread{\var}{1}$\\
% $\dots$
% \end{minipage}

% \caption{An infinite execution which is $B$-\cmp{}, but not 
% eventually linearizable}
% \label{fig:cmpnotel}

% \end{subfigure}


% \caption{
%     Histories showing the difference between $B$-\cmp{} and eventual
%     consistency.
% }
% \label{fig:allfigs}
% \end{figure} 


\begin{definition}[\cite{replicated-data-consistency-explained-through-baseball,cooper2008pnuts,viotti2015consistency}]
% Let $\bound: \Nat \rightarrow \Nat$ be a increasing function whose limit
% at $+\infty$ is $+\infty$.
Let $\bound \in \Nat$.
The history $\hist = (\ops,\po,\flabel)$ is 
\emph{$B$-\cmp{} (Consistent Monotonic Prefixes)} 
with respect to a specification $\spec$
if there exist a strict total order 
$\go \subseteq \ops \times \ops$ 
and a strict partial order $\vis \subseteq \ops \times \ops$ such that
for every $\op \in \ops$
there exists a sequence $\loco \in \spec$ satisfying
the axioms \axthinair, \axrv, \axmr,
\axbounded, 
\axprefix{} defined in 
\tab{tab:axioms}. 
\end{definition}

Axiom~\axthinair{} is due to physical constraints, as 
$\op_1 \ltrel{\vis} \op_2$ intuitively means that operation $\op_1$ is 
visible to operation $\op_2$.

Axiom~\axrv{} is a safety constraint, ensuring that the return value of $\op$
is valid according to the specification $\spec$. More specifically, it
ensures that the return value of $\op$ can be obtained by ordering the 
operations visible to $\op$ in some order which respects the specification 
$\spec$.

Formally, to define \axrv, we take the labelled poset $\thepast{\op}$, which
orders all the operations visible to $\op$ before $\op$ itself, and
project away all return values except $\op$'s.
We then verify that the resulting labelled poset, 
$\projectrv{\thepast{\op}}{\op}$,
can be sequentialized into a sequence $\loco$ of the specification, that is
$\projectrv{\thepast{\op}}{\op} \weaker \loco$.

Axiom~\axmr{} says that if $\op_1 \ltvis \op_2$, 
then $\op_1 \ltvis \op_3$ for all operations $\op_3$ with 
$\op_2 \ltpo \op_3$.
Intuitively, when a site $\pid$ becomes aware of an operation $\op_1$,
$\pid$ does not forget about $\op_1$.

% Axiom~\axbounded{} ensures that all operations are taken into account
% after at most $B$ rounds. 
% Note that \axbounded{} is weaker than 
% \axeventual.
Axiom~\axprefix{} ensures that each sequence $\loco$, for $\op \in \ops$
is a prefix of the global order $\go$.
% Axioms~\axbounded{} and \axprefix{} together imply \axeventual, leading
% to the following lemma.

% \begin{lemma}
% If a history $\hist = (\ops,\po,\flabel)$ has $B$-\cmp{} with respect
% to a specification $\spec$, then $\hist$ is $B$-\ec.
% \end{lemma}
% 
% \begin{proof}
% By definition, 
% there exist a strict total order 
% $\go \subseteq \ops \times \ops$ 
% and a strict partial order $\vis \subseteq \ops \times \ops$ such that
% for every $\op \in \ops$
% there exists a sequence $\loco \in \spec$ satisfying
% the axioms \axthinair, \axrv, 
% \axbounded, \axprefix{}. 
% 
% In particular, for each round $r \in \Nat$ and $\op \in \ops$ with
% $\getround(\op) > r + B$, we know
% $\getbefore{\ops}{r} \subseteq \loco$  and $\loco \pref \go$.
% This means that $\loco$ is a prefix of $\go$, and $\loco$ contains 
% all operations which happened at round $r$ or before.
% This implies that $\getprefix{\go}{r} \pref \loco$, so 
% axiom \axeventual{} is satisfied.
% 
% We conclude that $\hist$ is $B$-\ec.
% \end{proof}
% 
% \begin{lemma}
% There are histories which are $B$-\ec, but do not have $B$-\cmp.
% \end{lemma}
% 
% \begin{proof}
% site 1: wr(1) rd(2) rd(1)
% 
% site 2: wr(2) rd(1) rd(2)
% \end{proof}

\subsection{Comparison with other Consistency Criteria}

Eventual 
linearizability~\cite{Guerraoui:2014:PEL:2611462.2611484,serafini2010eventually}
is a consistency criterion which is not comparable to 
\cmp.
Informally, for an infinite execution $\exec$, eventual linearizability
ensures that there exists a point $p$ in $\exec$ after which the real-time
order is preserved. Operations before $p$ may be reordered.
Eventual linearizability is weaker than 
linearizability~\cite{journals/toplas/HerlihyW90}, 
as linearizability imposes that the real-time order is preserved
for the whole execution.

\fig{fig:elnotcmp} gives an execution $e_1$ which is
eventually linearizable but not $B$-\cmp{} (for any $B$).
Indeed, $e_1$ is eventually linearizable as we can say that the point $p$
is the end of the execution, allowing us to reorder the operations into
a valid sequence of reads and writes.

However, $e_1$ is not $B$-\cmp (for any $B$). 
Axioms~\axmr{} and \axprefix{} require that 
the last read operation of $p_a$ return value $2$, not $1$.

\fig{fig:cmpnotel} gives an execution $e_2$ which is $2$-\cmp{}, but is not 
eventually linearizable. Execution $e_2$ is $2$-\cmp{}, because even though
the reads do not return the last written value, they return a value
coming from a prefix of a global order $\go$, ordering the writes
as they appear in the execution (with a delay of $2$ rounds -- assuming
one operation per round).

Moreover, $e_2$ is not eventually linearizable, as the execution is 
infinite, and at no point in time do the operations respect the 
real-time order (no read returns the last written value to $\var$).
% Eventual linearizability is not comparable.
% (w(0) w(1) r(0) r(1))* has \cmp{} but is not eventually linearizable.


% site 1: wr(1) rd(2) rd(1)

% site 2: wr(2) rd(1) rd(2)
% is eventually linearizable but does not have \cmp{}

The definitions of eventual consistency given in 
\cite{Gotsman05,principles-of-eventual-consistency} and \cite{DBLP:conf/popl/BouajjaniEH14} are weaker than \cmp. 
In particular, they do not ensure axiom \axprefix,
and allow executions such as the one given in \fig{fig:elnotcmp}.
% do not guarantee the monotonic 
% 
% Eventual consistency of Burckhardt is weaker.
% They don't have monotonic reads over there!
% 
% site 1: wr(1) rd(1) rd(2) rd(1)
% 
% site 2: wr(2)
% 
% is ECB but doesn't have \cmp{}.


==> properties.tex <==
% % !TEX root = main.tex

% \begin{table}

% \begin{tabular}{ll}
% $\hasempty$     & $\emptyseq \in \gettrace{\semantics{\impl}}$  \\
% $\availability$ & 
%   $\forall \tr \in \gettrace{\semantics{\impl}}.\  
%   \forall \req \in \Req.\ 
%   \forall \pid \in \Pid.\ 
%   \exists \ans \in \Ans.\  
%   \tr \cdot (\pid,\req,ans) \in \gettrace{\semantics{\impl}}$ \\
% % $\writesymmetry$ &
% %   $
% %   \forall \pid \in \Pid.\
% %   \forall \pid\,' \in \Pid.\
% %   \forall n \in \Nat.\ 
% %   \forall \tr_1 \cdot (\pid,\mkwrite{n}) \cdot \tr_2 \in \gettrace{\semantics{\impl}}.$\\
% %   & \hspace{5em} 
% %   $\tr_1 \cdot (\pid\,',\mkwrite{n}) \cdot \tr_2 \in \gettrace{\semantics{\impl}}$ \\
% % $\commute$       &  
% %   $\forall \tr_1 \cdot \act_1 \cdot \act_2 \cdot \tr_2 \in \gettrace{\semantics{\impl}}.\
% %   [(\neg\isAppend(\act_1) \lor \neg\isRead(\act_2)) \land 
% %   \getPid(\act_1) \neq  \getPid(\act_2)]$ \\
% %   & \hspace{5em} $\implies 
% %     \tr_1 \cdot \act_2\ \cdot \act_1 \cdot \tr_2 \in \gettrace{\semantics{\impl}}$\\
% $\invisibleread$    & 
%   $\forall \tr_1 \cdot \act \cdot \tr_2 \in \gettrace{\semantics{\impl}}.\
%   \isRead(\act) \implies \tr_1 \cdot \tr_2 \in \gettrace{\semantics{\impl}}$ \\
% \end{tabular}
% \\
% \hspace{-40em}where:
% \begin{itemize} 
%   \item $\content(\ell) = \set{n \in \Nat\ |\ n \in \ell}$
%   \item $\appends(\tr) = \set{n \in \Nat\ |\ \append(n) \in \tr}$
% \end{itemize}

% \caption{Properties of Implementations}
% \label{tab:properties}

% \end{table}

% \ttodo{Rewrite these properties properties in terms of reads and writes.}
% \ttodo{Change $\hasempty$ and $\availability$ into lemmas.
% $\invisibleread$ is an extra assumption.}
